Delving into the Phenomenology of Very Special Relativity: From Subatomic Particles to Binary Stars

In this thesis, we investigate the implications of Lorentz-violating (LV) theories, focusing on Very Special Relativity (VSR) and its phenomenological consequences. Initially presented as an alternative mechanism for neutrino masses, VSR has since become a significant part of the general LV framework, distinguished by its unique group structure and non-local operators. After a comprehensive introduction to the principles of LV and VSR, we present the corresponding modifications to the Dirac equation. A significant part of the thesis is dedicated to the development of a Hamiltonian formalism within the VSR context, addressing its inherent non-localities. This approach is further extended to the non-relativistic limit, connecting it to the conventional Schr\"odinger picture. We then set upper bounds on the VSR parameters by examining its corrections to a wide range of physical systems and scenarios, such as Landau levels of charged particles, the $\mathsf g-$factor of electrons, the energy spectrum of ultracold neutrons in Earth's gravitational field, and the gravitational emission from binary stars. The latter analysis led us to the construction of a VSR field theory for spin-2 fields in flat space, which was surprisingly found to accommodate a gauge-invariant graviton mass. Through this comprehensive study, we bridged theoretical predictions with experimental data, paving the way for future explorations in Lorentz-violating theories and highlighting their potential to address unresolved questions in modern physics.

==> chapters/9_abbreviations.tex <==
\raggedright
\begin{itemize}
    \item LI $\,:\,$ \textit{Lorentz Invariance}
    \item QED $\,:\,$ \textit{Quantum Electrodynamics}
    \item SM $\,:\,$ \textit{Standard Model of Particles}
    \item QFT $\,:\,$ \textit{Quantum Field Theory}
    \item LT $\,:\,$ \textit{Lorentz Transformations}
    \item PLT $\,:\,$ \textit{Particle Lorentz Transformations}
    \item OLT $\,:\,$ \textit{Observer Lorentz Transformations}
    \item SR $\,:\,$ \textit{Special Relativity}
    
    \item GR $\,:\,$ \textit{General Relativity}
    \item VSR $\,:\,$ \textit{Very Special Relativity}
    \item QM $\,:\,$ \textit{Quantum Mechanics}
    \item EOM $\,:\,$ \textit{Equations of Motion}
    \item DOF $\,:\,$ \textit{Degrees of Freedom}
\end{itemize}

==> chapters/9_symbols.tex <==
\raggedright


$\partial$ $\;:\;$ Partial Derivatives \\
$D$ $\;:\;$ Covariant Derivatives \\
$\gamma$ $\;:\;$ Gamma Matrices \\
$\sigma$ $\;:\;$ Pauli Matrices \\

